TimeDRL: Disentangled Representation Learning for Multivariate Time-Series

Multivariate time-series data in numerous real-world applications (e.g., healthcare and industry) are informative but challenging due to the lack of labels and high dimensionality. Recent studies in self-supervised learning have shown their potential in learning rich representations without relying on labels, yet they fall short in learning disentangled embeddings and addressing issues of inductive bias (e.g., transformation-invariance). To tackle these challenges, we propose TimeDRL, a generic multivariate time-series representation learning framework with disentangled dual-level embeddings. TimeDRL is characterized by three novel features: (i) disentangled derivation of timestamp-level and instance-level embeddings from patched time-series data using a [CLS] token strategy; (ii) utilization of timestamp-predictive and instance-contrastive tasks for disentangled representation learning, with the former optimizing timestamp-level embeddings with predictive loss, and the latter optimizing instance-level embeddings with contrastive loss; and (iii) avoidance of augmentation methods to eliminate inductive biases, such as transformation-invariance from cropping and masking. Comprehensive experiments on 6 time-series forecasting datasets and 5 time-series classification datasets have shown that TimeDRL consistently surpasses existing representation learning approaches, achieving an average improvement of forecasting by 58.02% in MSE and classification by 1.48% in accuracy. Furthermore, extensive ablation studies confirmed the relative contribution of each component in TimeDRL's architecture, and semi-supervised learning evaluations demonstrated its effectiveness in real-world scenarios, even with limited labeled data. The code is available at https://github.com/blacksnail789521/TimeDRL.

==> Table/ablation_pretext_tasks.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Ablation study on pretext tasks.} We use the prediction length \(T = 168\) for ETTh1. The best results are in \textbf{bold}.}
\label{tab:ablation_pretext_tasks}
\begin{tblr}{
  rowsep = \myrowsep,
  % colsep = 5pt,
  cells={font=\small},
  cells = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=2}{},
  cell{1}{4} = {c=3}{},
  vline{2,4} = {-}{},
  hline{1,2,3,6} = {-}{},
}
Pretext Tasks & ETTh1 &  & FingerMovements &  & \\
 & MSE (\(\downarrow\)) & MAE (\(\downarrow\)) & ACC (\(\uparrow\)) & MF1 (\(\uparrow\)) & \(\kappa\) (\(\uparrow\))\\
TimeDRL & \textbf{0.418} & \textbf{0.427} & \textbf{63.00} & \textbf{63.00} & \textbf{26.06}\\
TimeDRL w/o
  Timestamp-Predictive & 0.423 (+1.2\%) & 0.430 (+0.58\%) & 56.00 (-11.11\%) & 56.00 (-11.11\%) & 12.04 (-53.8\%)\\
TimeDRL w/o
  Instance-Contrastive & 0.505 (+20.81\%) & 0.479 (+12.05\%) & 55.00 (-12.7\%) & 55.00 (-12.7\%) & 10.00 (-61.63\%)
\end{tblr}
\end{table*}
